Generalized Coordinated Multipoint Framework for 5G and Beyond

The characteristic feature of 5G is the diversity of its services for different user needs. However, the requirements for these services are competing in nature, which impresses the necessity of a coordinated and flexible network architecture. Although coordinated multipoint (CoMP) systems were primarily proposed to improve the cell edge performance in 4G, their collaborative nature can be leveraged to support the diverse requirements and enabling technologies of 5G and beyond networks. To this end, we propose generalization of CoMP to a proactive and efficient resource utilization framework capable of supporting different user requirements such as reliability, latency, throughput, and security while considering network constraints. This article elaborates on the multiple aspects, inputs, and outputs of the generalized CoMP (GCoMP) framework. Apart from user requirements, the GCoMP decision mechanism also considers the CoMP scenario and network architecture to decide upon outputs such as CoMP technique or appropriate coordinating clusters. To enable easier understanding of the concept, popular use cases, such as vehicle-to-everything (V2X) communication and eHealth, are studied. Additionally, interesting challenges and open areas in GCoMP are discussed.

==> AcronymList.tex <==
\usepackage{etoolbox}
\makeatletter
\newif\ifAC@uppercase@first%
\def\Aclp#1{\AC@uppercase@firsttrue\aclp{#1}\AC@uppercase@firstfalse}%
\def\AC@aclp#1{%
	\ifcsname fn@#1@PL\endcsname%
	\ifAC@uppercase@first%
	\expandafter\expandafter\expandafter\MakeUppercase\csname fn@#1@PL\endcsname%
	\else%
	\csname fn@#1@PL\endcsname%
	\fi%
	\else%
	\AC@acl{#1}s%
	\fi%
}%
\def\Acp#1{\AC@uppercase@firsttrue\acp{#1}\AC@uppercase@firstfalse}%
\def\AC@acp#1{%
	\ifcsname fn@#1@PL\endcsname%
	\ifAC@uppercase@first%
	\expandafter\expandafter\expandafter\MakeUppercase\csname fn@#1@PL\endcsname%
	\else%
	\csname fn@#1@PL\endcsname%
	\fi%
	\else%
	\AC@ac{#1}s%
	\fi%
}%
\def\Acfp#1{\AC@uppercase@firsttrue\acfp{#1}\AC@uppercase@firstfalse}%
\def\AC@acfp#1{%
	\ifcsname fn@#1@PL\endcsname%
	\ifAC@uppercase@first%
	\expandafter\expandafter\expandafter\MakeUppercase\csname fn@#1@PL\endcsname%
	\else%
	\csname fn@#1@PL\endcsname%
	\fi%
	\else%
	\AC@acf{#1}s%
	\fi%
}%
\def\Acsp#1{\AC@uppercase@firsttrue\acsp{#1}\AC@uppercase@firstfalse}%
\def\AC@acsp#1{%
	\ifcsname fn@#1@PL\endcsname%
	\ifAC@uppercase@first%
	\expandafter\expandafter\expandafter\MakeUppercase\csname fn@#1@PL\endcsname%
	\else%
	\csname fn@#1@PL\endcsname%
	\fi%
	\else%
	\AC@acs{#1}s%
	\fi%
}%
\edef\AC@uppercase@write{\string\ifAC@uppercase@first\string\expandafter\string\MakeUppercase\string\fi\space}%
\def\AC@acrodef#1[#2]#3{%
	\@bsphack%
	\protected@write\@auxout{}{%
		\string\newacro{#1}[#2]{\AC@uppercase@write #3}%
	}\@esphack%
}%
\def\Acl#1{\AC@uppercase@firsttrue\acl{#1}\AC@uppercase@firstfalse}
\def\Acf#1{\AC@uppercase@firsttrue\acf{#1}\AC@uppercase@firstfalse}
\def\Ac#1{\AC@uppercase@firsttrue\ac{#1}\AC@uppercase@firstfalse}
\def\Acs#1{\AC@uppercase@firsttrue\acs{#1}\AC@uppercase@firstfalse}
\robustify\Aclp
\robustify\Acfp
\robustify\Acp
\robustify\Acsp
\robustify\Acl
\robustify\Acf
\robustify\Ac
\robustify\Acs
\makeatother

\acrodef{PDCP}[PDCP]{packet data convergence protocol}
\acrodef{RATs}[RATs]{radio access technologies}
% \acrodefplural{RAT}[RAT]{radio access technologies}
\acrodef{AP}[AP]{access point}
\acrodef{MP-TCP}[MP-TCP]{Multipath transmission control protocol}
\acrodef{5QI}[5QI]{\ac{5G} \ac{QoS} identifier}
\acrodef{NSI}[NSI]{network slice instance}
\acrodef{ATSSS}[ATSSS]{access traffic steering, switching and splitting}
\acrodef{CA}[CA]{coordination area}
\acrodef{TRP}[TRP]{transmission-reception point}
\acrodef{SON}[SON]{self-organizing network}
\acrodef{V2X}[V2X]{vehicle-to-everything}
\acrodef{eMBB}[eMBB]{enhanced mobile broadband}
\acrodef{mMTC}[mMTC]{massive machine type communication}
\acrodef{uRLLC}[uRLLC]{ultra-reliable low latency communication}
\acrodef{CoMP}[CoMP]{coordinated multipoint}
\acrodef{LTE}[LTE]{Long Term Evolution}
\acrodef{LTE-A}[LTE-A]{LTE-Advanced}
\acrodef{3GPP}[3GPP]{3rd Generation Partnership Project}
\acrodef{FFR}[FFR]{fractional frequency reuse}
\acrodef{SFR}[SFR]{soft frequency reuse}
\acrodef{ICI}[ICI]{inter-cell interference}
\acrodef{ICIC}[ICIC]{inter-cell interference coordination}
\acrodef{eICIC}[eICIC]{enhanced \ac{ICIC}}
\acrodef{ABS}[ABS]{absolute blank subframe}
\acrodef{TP}[TP]{transmission point}
\acrodef{CSI}[CSI]{channel state information}
\acrodef{eNB}[eNB]{eNodeB}
\acrodef{RAN}[RAN]{radio access network}
\acrodef{C-RAN}[C-RAN]{cloud-RAN}
\acrodef{RRH}[RRH]{remote radio head}
\acrodef{BBU}[BBU]{baseband unit}
\acrodef{CS}[CS]{coordinated scheduling}
\acrodef{CB}[CB]{coordinated beamforming}
\acrodef{JT}[JT]{joint transmission}
\acrodef{NC-JT}[NC-JT]{non-coherent \ac{JT}}
\acrodef{C-JT}[C-JT]{coherent \ac{JT}}
\acrodef{DPS}[DPS]{dynamic point selection}
\acrodef{TTI}[TTI]{transmission time interval}
\acrodef{UE}[UE]{user equipment}
\acrodef{RNTP}[RNTP]{relative narrowband transmission power}
\acrodef{eRNTP}[eRNTP]{enhanced \ac{RNTP}}
\acrodef{OI}[OI]{overload indicator}
\acrodef{HII}[HII]{high interference indicator}
\acrodef{HG}[HG]{Hermite-Gaussian}
\acrodef{CQI}[CQI]{channel quality indicator}
\acrodef{PMI}[PMI]{precoding matrix indicator}
\acrodef{RI}[RI]{rank indicator}
\acrodef{HetNet}[HetNet]{heterogeneous network}
\acrodef{mmWave}[mmWave]{millimeter wave}
\acrodef{SINR}[SINR]{signal-to-interference-plus-noise ratio}
\acrodef{SC}[SC]{single-carrier}
\acrodef{SM-OFDM}[SM-OFDM]{Spatial modulation-OFDM}
\acrodef{GB}[GB]{guard band}
\acrodef{DL}[DL]{downlink}
\acrodef{FFT}[FFT]{fast Fourier transform}
\acrodef{IFFT}[IFFT]{inverse fast Fourier transform}
\acrodef{CP}[CP]{cyclic prefix}
\acrodef{GBR}[GBR]{guaranteed bit-rate}
\acrodef{GFDM}[GFDM]{generalized orthogonal frequency division multiplexing}
\acrodef{RSRP}[RSRP]{reference signal received power}
\acrodef{CSI-RSRP}[CSI-RSRP]{CSI-reference signal received power}
\acrodef{se}[SE]{spectral efficiency}
\acrodef{5G}[5G]{fifth generation}
\acrodef{4G}[4G]{fourth generation}
\acrodef{papr}[PAPR]{peak-to-average power ratio}
\acrodef{isi}[ISI]{intersymbol interference}
\acrodef{wdm}[WDM]{waveform division multiplexing}
\acrodef{noma}[NOMA]{non-orthogonal multiple access}
\acrodef{MIMO}[MIMO]{multiple-input multiple-output}
\acrodef{GCoMP}[GCoMP]{generalized CoMP}
\acrodef{CU}[CU]{central unit}
\acrodef{DU}[DU]{distributed unit}
\acrodef{RU}[RU]{remote unit}
\acrodef{FH}[FH]{fronthaul}
\acrodef{LoS}[LoS]{line-of-sight}
\acrodef{TBS}[TBS]{terrestrial base station}
\acrodef{FBS}[FBS]{flying base station}
\acrodef{pls}[PLS]{physical layer security}
\acrodef{PRB}[PRB]{physical resource block}
\acrodef{PSK}[PSK]{phase-shift keying}
\acrodef{QAM}[QAM]{quadrature amplitude modulation}
\acrodef{ostbc}[OSTBC]{orthogonal space time block codes}
\acrodef{OOBE}[OOBE]{out-of-band emission}
\acrodef{svd}[SVD]{singular value decomposition}
\acrodef{MAC}[MAC]{medium access control}
\acrodef{PHY}[PHY]{physical}
\acrodef{THz}[THz]{terahertz}
\acrodef{RIS}[RIS]{reconfigurable intelligent surface}
\acrodef{QoS}[QoS]{quality of service}
\acrodef{ITS}[ITS]{intelligent transportation system}
% \acrodef{TRxP}[TRxP]{transmission reception point}
\acrodef{HO}[HO]{handover}
\acrodef{TUBITAK}[TUBITAK]{Scientific and Technological Research Council of Turkey}
\acrodef{MBB}[MBB]{\textit{Make-Before-Break}}
\acrodef{RACH}[RACH]{\textit{Random Access Channel}}
\acrodef{eMTC}[eMTC]{\textit{enhanced machine type communication}}
